POp-GS: Next Best View in 3D-Gaussian Splatting with P-Optimality

In this paper, we present a novel algorithm for quantifying uncertainty and information gained within 3D Gaussian Splatting (3D-GS) through P-Optimality. While 3D-GS has proven to be a useful world model with high-quality rasterizations, it does not natively quantify uncertainty or information, posing a challenge for real-world applications such as 3D-GS SLAM. We propose to quantify information gain in 3D-GS by reformulating the problem through the lens of optimal experimental design, which is a classical solution widely used in literature. By restructuring information quantification of 3D-GS through optimal experimental design, we arrive at multiple solutions, of which T-Optimality and D-Optimality perform the best quantitatively and qualitatively as measured on two popular datasets. Additionally, we propose a block diagonal covariance approximation which provides a measure of correlation at the expense of a greater computation cost.

==> template/Definitions.tex <==
\usepackage{graphicx}
\usepackage{caption, subcaption}
\captionsetup{size=footnotesize,
    %justification=centering, %% not needed
    skip=5pt, position = bottom}
\usepackage{amsmath,amssymb,enumerate}
\let\proof\relax 
\let\endproof\relax
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{breqn}
\usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
% \usepackage[colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed]{hyperref}
\usepackage{algorithm, algpseudocode}
\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$~\textcolor{Gray}{#1}}
\usepackage{blindtext}
\usepackage{gensymb}
\usepackage{bm}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{times}
 \usepackage{amsmath}
% \usepackage[noadjust]{cite} % to group references
% \usepackage[numbers,sort&compress]{natbib}
% \usepackage{multicol}
% \usepackage[caption=false,font=normalsize]{subfig}
% \usepackage{amsfonts}
% \usepackage{cleveref}
% \usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage{balance}
\usepackage{soul}
\usepackage{multirow}
\usepackage{booktabs}
% \usepackage{wrapfig,lipsum,booktabs}
% \usepackage{wrapfig}
\usepackage{sidecap}
\usepackage{makecell}
\usepackage{array,float}
\usepackage{tabularx}

\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}}

\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\minimize}{minimize}
\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
\renewcommand{\thefigure}{\arabic{figure}}

\newcommand{\mgj}[1]{[{\textbf{\textcolor{BrickRed}{Maani: #1}}}]}
\newcommand{\squeezeup}{\vspace{-3mm}}
\newcommand{\prompt}[1]{[{\emph{\textbf{\textcolor{ForestGreen}{#1 }}}}]}
\newcommand{\rough}[1]{[{\emph{\textbf{\textcolor{Blue}{#1 }}}}]}
\newcommand{\todojoey}[1]{[{\emph{\textbf{\textcolor{Red}{Joey (TODOs): #1}}}}]}
\newcommand{\jw}[1]{[{\textbf{\textcolor{Red}{Joey: #1}}}]}
\newcommand{\jy}[1]{[{\textbf{\textcolor{Blue}{Jingyu: #1}}}]}
\newcommand{\az}[1]{[{\textbf{\textcolor{Green}{Arthur: #1}}}]}
\newcommand{\yf}[1]{[{\textbf{\textcolor{Orange}{Yuewei: #1}}}]}

%\usepackage[ruled]{algorithm2e} % http://www.ctan.org/pkg/algorithm2e

\definecolor{free}{rgb}{0.9608, 0.5882, 0.3922}
\definecolor{building}{rgb}{0.9608, 0.9020, 0.3922}
\definecolor{barrier}{rgb}{0.5882, 0.2353, 0.1176}
\definecolor{other}{rgb}{0.7059, 0.1176, 0.3137}
\definecolor{pedestrian}{rgb}{1, 0.3137, 0.3922}
\definecolor{pole}{rgb}{0.1176, 0.1176, 1}
\definecolor{road}{rgb}{0.7843, 0.1569, 1}
\definecolor{ground}{rgb}{0.3529, 0.1176, 0.5882}
\definecolor{sidewalk}{rgb}{1, 0, 1}
\definecolor{vegetation}{rgb}{1, 0.5882, 1}
\definecolor{vehicles}{rgb}{0.2941, 0, 0.2941}
\definecolor{fence}{rgb}{0.1961, 0.4706, 1}
\definecolor{sign}{rgb}{0, 0, 1}


\definecolor{scarColor}{rgb}{0.9608, 0.5882, 0.3922}
\definecolor{sbicycleColor}{rgb}{0.2608, 0.9020, 0.3922}
\definecolor{smotorcycleColor}{rgb}{0.5882, 0.2353, 0.1176}
\definecolor{struckColor}{rgb}{0.7059, 0.1176, 0.3137}
\definecolor{sothervehicleColor}{rgb}{1, 0.3137, 0.3922}
\definecolor{spersonColor}{rgb}{0.1176, 0.1176, 1}
\definecolor{sbicyclistColor}{rgb}{0.7843, 0.1569, 1}
\definecolor{smotorcyclistColor}{rgb}{0.3529, 0.1176, 0.5882}
\definecolor{sroadColor}{rgb}{0.5, 0, 1}
\definecolor{sparkingColor}{rgb}{1, 0.5882, 1}
\definecolor{ssidewalkColor}{rgb}{0.2941, 0, 0.2941}
\definecolor{sothergroundColor}{rgb}{0.2941, 0, 0.6863}
\definecolor{sbuildingColor}{rgb}{0, 0.7843, 1}
\definecolor{sfenceColor}{rgb}{0.1961, 0.4706, 1}
\definecolor{svegetationColor}{rgb}{0, 0.6863 ,0}
\definecolor{strunkColor}{rgb}{0, 0.2353, 0.5294}
\definecolor{sterrainColor}{rgb}{0.3137, 0.9412, 0.5882}
\definecolor{spoleColor}{rgb}{0.5882, 0.7412, 1}
\definecolor{strafficsignColor}{rgb}{0, 0, 1}


% \newcommand{\RKHS}{\Hcal_k}
% %\renewcommand{\g}{\mathfrak{g}}
% % \DeclareMathOperator{\SE}{SE}
% \DeclareMathOperator{\diff}{Diff}
% % \DeclareMathOperator{\SO}{SO}
% \DeclareMathOperator{\tr}{Tr}
% \DeclareMathOperator{\Lie}{Lie}
% \newcommand{\se}{\mathfrak{se}}
% % \newcommand{\so}{\mathfrak{so}}
% \newcommand{\I}{\mathcal{I}}
% \newcommand{\sumxz}{\sum_{\substack{x_i\in X\\ z_j\in Z}}}

\newcommand{\bigO}[1]{\Ocal(#1)} % Big O
\newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
\newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
\newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance

\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\m}{\mathop{\mathrm{m}}}
\newcommand{\rad}{\mathop{\mathrm{rad}}}
\newcommand{\dBm}{\mathop{\mathrm{dBm}}}
\newcommand{\Hz}{\mathop{\mathrm{Hz}}}
\newcommand{\GHz}{\mathop{\mathrm{GHz}}}
\newcommand{\MHz}{\mathop{\mathrm{MHz}}}

% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
% \newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
% \newcommand{\Fcal}{\mathcal{F}}
% \newcommand{\Gcal}{\mathcal{G}}
% \newcommand{\Hcal}{\mathcal{H}}
% \newcommand{\Ical}{\mathcal{I}}
% \newcommand{\Kcal}{\mathcal{K}}
% \newcommand{\Lcal}{\mathcal{L}}
% \newcommand{\Mcal}{\mathcal{M}}
% \newcommand{\Ncal}{\mathcal{N}}
% \newcommand{\Ocal}{\mathcal{O}}
% \newcommand{\Scal}{\mathcal{S}}
% \newcommand{\Xcal}{\mathcal{X}}
% \newcommand{\Ycal}{\mathcal{Y}}
% \newcommand{\Zcal}{\mathcal{Z}}

% \newcommand{\Exp}{\mathrm{Exp}}
% \newcommand{\Log}{\mathrm{Log}}
% \newcommand{\Jr}{\mathrm{J_r}}
\newcommand{\transpose}{\mathsf{T}}
% \newcommand{\SO}{\mathrm{SO}}
% \newcommand{\SE}{\mathrm{SE}}
% \newcommand{\GL}{\mathrm{GL}}



% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
%\DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}
